DB-LSH: Locality-Sensitive Hashing with Query-based Dynamic Bucketing

Among many solutions to the high-dimensional approximate nearest neighbor (ANN) search problem, locality sensitive hashing (LSH) is known for its sub-linear query time and robust theoretical guarantee on query accuracy. Traditional LSH methods can generate a small number of candidates quickly from hash tables but suffer from large index sizes and hash boundary problems. Recent studies to address these issues often incur extra overhead to identify eligible candidates or remove false positives, making query time no longer sub-linear. To address this dilemma, in this paper we propose a novel LSH scheme called DB-LSH which supports efficient ANN search for large high-dimensional datasets. It organizes the projected spaces with multi-dimensional indexes rather than using fixed-width hash buckets. Our approach can significantly reduce the space cost as by avoiding the need to maintain many hash tables for different bucket sizes. During the query phase of DB-LSH, a small number of high-quality candidates can be generated efficiently by dynamically constructing query-based hypercubic buckets with the required widths through index-based window queries. For a dataset of $n$ $d$-dimensional points with approximation ratio $c$, our rigorous theoretical analysis shows that DB-LSH achieves a smaller query cost ${O(n^{\rho^*} d\log n)}$, where ${\rho^*}$ is bounded by ${1/c^{\alpha}}$ while the bound is ${1/c}$ in the existing work. An extensive range of experiments on real-world data demonstrates the superiority of DB-LSH over state-of-the-art methods on both efficiency and accuracy.

==> expe_n.tex <==
 \begin{figure}[t]
    \begin{minipage}[c]{0.8\linewidth}
		\centering
		\includegraphics[width=.7\textwidth]{expe/legend_short}
		\vspace{1em}
	\end{minipage}
 	\centering
 	\subfigure[Gist]{
 		\begin{minipage}[c]{0.45\linewidth}
 			\centering
 			\includegraphics[width=1\textwidth]{expe/gist_n_time}
 			\vspace{-1em}
 		\end{minipage}
 	}
 	\subfigure[TinyImages80M]{
 		\begin{minipage}[c]{0.45\linewidth}
 			\centering
 			\includegraphics[width=1\textwidth]{expe/tiny_n_time.pdf}
 			\vspace{-1em}
 		\end{minipage}
 	}
 	\vspace{-0.5em}\caption{Query Time when Varying $n$}\vspace{-1em}
 	\label{expe:n_time}
 \end{figure}
 \begin{figure}[t]
 	\centering
 	\subfigure[Gist]{
 		\begin{minipage}[c]{0.45\linewidth}
 			\centering
 			\includegraphics[width=1\textwidth]{expe/gist_n_recall.pdf}
 			\vspace{-1em}
 		\end{minipage}
 	}
 	\subfigure[TinyImages80M]{
 		\begin{minipage}[c]{0.45\linewidth}
 			\centering
 			\includegraphics[width=1\textwidth]{expe/tiny_n_recall.pdf}
 			\vspace{-1em}
 		\end{minipage}
 	}
 	\vspace{-0.5em}\caption{Recall when Varying $n$}\vspace{-1em}
 	\label{expe:n_recall}
 \end{figure}
 \begin{figure}[H]
 	\centering
 	\subfigure[Gist]{
 		\begin{minipage}[c]{0.45\linewidth}
 			\centering
 			\includegraphics[width=1\textwidth]{expe/gist_n_ratio.pdf}
 			\vspace{-1em}
 		\end{minipage}
 	}
 	\subfigure[TinyImages80M]{
 		\begin{minipage}[c]{0.45\linewidth}
 			\centering
 			\includegraphics[width=1\textwidth]{expe/tiny_n_ratio.pdf}
 			\vspace{-1em}
 		\end{minipage}
 	}
 	\vspace{-0.5em}\caption{Overall Ratio when Varying $n$} \vspace{-1em}
 	\label{expe:n_ratio}
 \end{figure}
 
 
%\begin{figure}
%	\begin{minipage}[c]{0.8\linewidth}
%		\centering
%		\includegraphics[width=.7\textwidth]{expe/legend_short}
%		\vspace{0.5em}
%	\end{minipage}
%	\begin{minipage}[t]{\linewidth}
%		\centering
%		\subfigure[Gist]{
%			\begin{minipage}[c]{0.45\linewidth}
%				\centering
%				\includegraphics[width=1\textwidth]{expe/gist_n_time}
%				\vspace{-1em}
%			\end{minipage}
%		}
%		\subfigure[TinyImages80M]{
%			\begin{minipage}[c]{0.45\linewidth}
%				\centering
%				\includegraphics[width=1\textwidth]{expe/tiny_n_time.pdf}
%				\vspace{-1em}
%			\end{minipage}
%		}
%		\caption{Query Time when Varying $n$}
%		\label{expe:n_time}
%	\end{minipage}%
%	\begin{minipage}[t]{\linewidth}
%		\centering
%		\subfigure[Gist]{
%			\begin{minipage}[c]{0.45\linewidth}
%				\centering
%				\includegraphics[width=1\textwidth]{expe/gist_n_recall.pdf}
%				\vspace{-1em}
%			\end{minipage}
%		}
%		\subfigure[TinyImages80M]{
%			\begin{minipage}[c]{0.45\linewidth}
%				\centering
%				\includegraphics[width=1\textwidth]{expe/tiny_n_recall.pdf}
%				\vspace{-1em}
%			\end{minipage}
%		}
%		\caption{Recall when Varying $n$}
%		\label{expe:n_recall}
%	\end{minipage}
%\end{figure}
 %\begin{figure*}[htbp]
%	\centering
%	\subfigure[Time]{
%		\begin{minipage}[c]{0.3\linewidth}
%			\centering
%			\includegraphics[width=1\textwidth]{expe/gist_n_time.pdf}
%		\end{minipage}
%	}
%	\subfigure[Recall]{
%		\begin{minipage}[c]{0.3\linewidth}
%			\centering
%			\includegraphics[width=1\textwidth]{expe/gist_n_recall.pdf}
%		\end{minipage}
%	}
%	\subfigure[OverRatio]{
%		\begin{minipage}[c]{0.3\linewidth}
%			\centering
%			\includegraphics[width=1\textwidth]{expe/gist_n_ratio.pdf}
%		\end{minipage}
%	}
%	\caption{Performance on Gist when Varying $n$}
%	\label{expe:n_gist}
%\end{figure*}
%
%\begin{figure*}[htbp]
%	\centering
%	\subfigure[Time]{
%		\begin{minipage}[c]{0.3\linewidth}
%			\centering
%			\includegraphics[width=1\textwidth]{expe/tiny_n_time.pdf}
%		\end{minipage}
%	}
%	\subfigure[Recall]{
%		\begin{minipage}[c]{0.3\linewidth}
%			\centering
%			\includegraphics[width=1\textwidth]{expe/tiny_n_recall.pdf}
%		\end{minipage}
%	}
%	\subfigure[OverRatio]{
%		\begin{minipage}[c]{0.3\linewidth}
%			\centering
%			\includegraphics[width=1\textwidth]{expe/tiny_n_ratio.pdf}
%		\end{minipage}
%	}
%	\caption{Performance on TinyImages80M when Varying $n$}
%	\label{expe:n_tiny}
%\end{figure*}

==> motivation.tex <==
\section{motivation}
\label{motivation}


E2LSH is a seminal solution for ANN search problem. As proven in xx,  by cleverly setting $K = \log_{1/p_2}n$ and $L = 1/p_1^{K}$, E2LSH can directly solve  $(r, c)$-NN problem with a constant success probability. Then the $c$-ANN query is also solved by multiple rounds of $(r, c)$-NN queries.
As shown in Table \ref{tb:comp_ATF_alg}, among existing solutions to $c$-ANN search problem, E2LSH is the only one that truly achieves sub-linear query cost, which means a great scalability potential  to large datasets. 
Although it has been put aside for years due to some difficulties, we argue that such simple and creative idea should not be abandoned yet.


\begin{comment}

Unfortunately, it is laid aside and neglect due to three drawbacks, \ie large index sizes, hash boundary problem and 
\begin{itemize}
    \item \textit{large index sizes.} Since it is difficult to design a perfect $K$-dimensional hash table such that every pair of close objects can fall in the same bucket, $L$ is usually large in order to guarantee a high accuracy. In addition, multiple sets of $(K, L)$-indexes for $(r, c)$-NN queries with different $r$ must be created in advance, which leads to expensive space cost potentially. 
    \item \textit{hash boundary problem.} Bucketing is completed in the pre-processing phase. When the query is close to the bucket boundary,  which makes it possible for points close to the query to be divided into different buckets.
    \item \textit{determining proper bucket width is non-trivial.}
\end{itemize}

\end{comment}

%\subsection{How to reduce index size?}
%\subsection{A one-size-fits-all $(K, L)$-Indexing?}
\subsection{How to design a one-size-fits-all $(K, L)$-Index?}

The first obstacle to answer the $c$-ANN problem using the $(K,L)$-indexing methods is the need to prepare a $(K, L)$-index for each $(r, c)$-NN where $r = 1, c, c^2, \ldots$, and $L$ in each suit is usually large, which incurs undesirable space and query costs. LSB \cite{DBLP:conf/sigmod/TaoYSK09} alleviates the first issue to some extents. Briefly, it builds a $(K, L)$-Index for $(1, c)$-NN and keeps merging small hash buckets into a large one, which in effect amounts to enlarging $r$. However, LSB only works for $(r,c)$-NN queries at some discrete integer $r$, which further causes LSB cannot answer $c$-ANN query with $c$ less than $4$. 
Designing  a $(K, L)$-Index that works with any  $r \geq 1$ ($c \geq 1$) remains to be a challenge.  
Our DM-LSH provides such `one-size-fits-all' $(K, L)$-Index, which removes the limitation of $r$ completely. Besides, by introducing a `magic' $t$, DM-LSH also reduces $L$.

% the query time and space complexities are directly proportional to the number of indexes, $L$.
% multiple suits for different radius $\rightarrow$ single suit for all radius
% but existing methods suffer from integer approximation ratio

\subsection{What is an appropriate bucket?}
An `appropriate' bucket is twofold. First, the bucket contains
as few false positives as possible. Second, points in the bucket can be retrieved quickly. 
E2LSH achieves fast retrieval by looking up hash tables, but it is subject to the hash boundary problem as mentioned earlier.
%that points close to the query are partitioned into different buckets, especially when the query is near the bucket boundary. 
Recent works adopt query-centric buckets. Such bucketing increases the probability of true positives, but it sacrifices retrieval efficiency, \ie query cost of these methods is no longer sub-linear with the cardinality. 

For example,  the search space of DC2 is an unbounded crossroad-like region when the threshold $l = 1$, \ie all points falling into this region are needed to be checked, which greatly damages the query performance. The blue circle in Figure X is the  search region defined in DMQ. In spite of ..., which is inherently time-consuming.

It is difficult to achieve a better balance between quality and efficiency. In DW-LSH, we adopt query-centric hypercubes as buckets on top of $(K, L)$-Indexing and introduce window query based searching strategy, which  enables DW-LSH to answer $c$-ANN problem in sub-linear time. 

%However, by analyzing search strategies from a geometric point of view, 
%Taking these two factors into consideration, DW-LSH adopts the query-centric hyper-cube is an appropriate bucket since it not only eliminates the bad effect of hash boundary but is easier to be worked out than the buckets of DC2 and DMQ. More importantly, the query-centric hyper-cube is compatible with $(K, L)$-Indexing, which enables DW-LSH to answer $c$-ANN problems in sub-linear query time.

% we find a smaller overhead can be achieved with out jeopardise candidates quality by conducting dynamic window queries. As illustrated in Figure X 


%  a  new  balance between   efficiency   and   cost   with   quality   guarantee. This observation inspires us to design dynamic(K,L)-Indexing by


% but existing methods suffer from unbounded search region, as shown in Figure X

\subsection{How to pursue a really bounded $\rho$?}
A strength of $(K,L)$-indexing methods is that its query cost is $O(dn^\rho\log_{1/p_2}n)$ and $\rho$ is theoretically bounded by ${1/c}$, \ie sub-linear query time. 
However, it is just a beautiful theory, since $1/c$ can be taken only if the bucket width $w$ tends to infinity \cite{DBLP:conf/compgeom/DatarIIM04}. Such large $w$ is nonsense in practice. 
Therefore, finding a smaller and actually bounded $\rho$ that can be used experimentally remains a challenge. As will shown in Section X, DW-LSH achieves a smaller $\rho$ bounded by \cred{$1/c^2$} at $w=4c^2$.

%It is always great to see cases where beautiful theory produces great results in practice.
%A really bounded and smaller $\rho$ not only benefits the quality guarantee but provides a better guidance for the experiments.
% Even though the dynamic $(K,L)$-indexing method can answer $(r,c)$-NN queries at any radius $r$ by only one framework, the number of required indexes, $L$, is still undesirable for quality guarantee.
% it’s always great to see cases where beautiful theory produces great results in practice.
% it's difficult to set bucket width
% Traditional methods $\rightarrow$ theory: infinity, but it's unpractical 
% Machine learning based methods $\rightarrow$ black box, no theoretical guarantee
% we need to propose a way to determine width such that both 1) practical and 2) theoretical guarantee (better than before)

\begin{comment}

\subsection{aaa}
To motivate our work, we analyze why using dynamic bucketing instead of static bucketing is capable of reviving $(K,L)$-indexing methods. As mentioned earlier, E2LSH, the classic $(K,L)$-indexing method, suffers from some stubborn shortcomings, such as hash boundary and unscalability, which limit its usage. Dynamic bucketing eliminates these two shortcomings fundamentally. 
Since the search region of the dynamic bucketing in the projected space is always centered at $q$, it is capable of being an optimal "bucket" no matter where the query point is located, which avoids the bad effect of hash boundary. 
%The collision probability of the close points increases a lot compared to that in the static bucketing methods. Although the collision probability of the far points also increases, we observe that $\rho$ becomes much smaller and the number of indexes for dynamic window query strategy reduces greatly. 
In addition, since no fixed bucket is required again, we use a data structure that supports window query instead of the hash table as our hash index, which enables us to answer $(r,c)$-NN queries at any radius $r$ by only one framework.

However, before designing a dynamic $(K,L)$-indexing method, the following two problems need to be well solved ahead.

%simply changing the window size of our window query. Therefore, it naturally supports to answer $c$-ANNS query with any approximation ratio by only one index framework. 
%Since so many obvious benefit does dynamic window query have, one would doubt why no work has adopted this strategy on bucketing methods. The challenges in using dynamic window query come from following aspects.

%However, two dynamic query strategies, DC2 and DMQ, have been proposed to improve E2LSH. Their tremendous advantages compared to E2LSH appeal to many researchers and numerous excellent methods come forth. Thus, it is challenging to design a $(K,L)$-indexing method that is comparable to the advanced LSH methods. Before designing a dynamic $(K,L)$-indexing method, the following two problems need to be well solved ahead.
%These new frameworks outperform the static bucketing methods and 
\begin{itemize}[leftmargin=*]
    \item Finding the points in the dynamic bucket is more time-consuming than accessing the static hash bucket.
    \item Even though the dynamic $(K,L)$-indexing method can answer $(r,c)$-NN queries at any radius $r$ by only one framework, the number of required indexes, $L$, is still undesirable for quality guarantee.
\end{itemize}

\subsection{Is the window query really too expensive to be answered?}
\textbf{1.}

Admittedly, answering a window query is obviously more time-consuming than pinpointing one or several hash buckets. Fortunately, the methods of efficiently answering a window query have been intensively studied \cite{1,2}. Among these methods, R*-Tree has a superior performance and is a good choice for answering the window query in low-dimensional space. We then adopt the in-memory R*-Tree as our index.

\textbf{2.}

windows query v.s. C2/Range query
Figure
To demonstrate that window query enables bucketing methods to be comparable with other dynamic LSH methods, we analyze the advantages of the Window-LSH over these methods.

When comparing to the collision counting based methods, Window-LSH has a smaller search region to obtain a certain number of candidates. As illustrated in the Fig. \ref{}, the search regions of the collision counting based methods are the union of several pillar-like regions unenclosed in $m-1$ dimensions. This kind of regions make the number of points access arbitrarily large in the worst case and thus lead to a large query cost. On contrary, the search regions of Window-LSH is $L$ enclosed hyper-cubes. The query cost of searching these regions are bounded.

As for metric query based methods, we need to conduct the exact nearest neighbor query in the projected space. In spite of the fact that the candidates obtained by this approach is best than other strategies \cite{DBLP:journals/pvldb/ZhengZWHLJ20}, it is inherently more expensive than answering window query at the same selectivity.

\subsection{Comparison with the other dynamic LSH methods}


%\subsection{Why R*-Tree?}
%\cred{\textbf{Find a paper on In-memory R*-Tree if using it.}}
% To ensure the efficiency of our method in finding candidate points, choosing a data structure as index that performs well for answering window query in low-dimensional space is necessary. In last few years, an ocean of learned indexes are designed, many of which is optimized for answering window query in low-dimensional space. However, the goal of their optimization is mainly to reduce the number of page access. Compared to the traditional indexes, such as R*-Tree and its variants, they have no advantage in terms of CPU time \cite{DBLP:conf/sigmod/Li0ZY020}. In addition, the query performance of these learned indexes degrades drastically with the increasing of data dimensionality.
% As we can see from their experiments \cred{\cite{1}}, R*-Tree has a superior performance and is a good choice for answering the window query in low-dimensional space.
% Therefore, we adopt the in-memory R*-Tree as our index \cite{DBLP:conf/ssd/HwangKCL03}.

% R*-Tree ....

% Note that R-Tree and R*-Tree have many variants, such as CR*-Tree, Hilbert R-Tree and so on. Study in \cite{DBLP:conf/ssd/HwangKCL03} showed that these variants perform better than R*-Tree when answering window query in some cases. However, since R*-Tree is one of the most popular spatial indexes, many optimizations and toolboxes have been built and maintained for R*-Tree, which enables R*-Tree to perform better practically. 


\end{comment}

